DeepPlace: Learning to Place Applications in Multi-Tenant Clusters

Large multi-tenant production clusters often have to handle a variety of jobs and applications with a variety of complex resource usage characteristics. It is non-trivial and non-optimal to manually create placement rules for scheduling that would decide which applications should co-locate. In this paper, we present DeepPlace, a scheduler that learns to exploits various temporal resource usage patterns of applications using Deep Reinforcement Learning (Deep RL) to reduce resource competition across jobs running in the same machine while at the same time optimizing for overall cluster utilization.

==> sec_conclusions.tex <==
\vspace{-1.8em}
\section{Conclusion}
\vspace{-1em}
We show an early design prototype of a self-learning scheduler that can exploit the temporal resource usage patterns and arrival dependencies of the jobs to provide a better placement policy and achieve better utilization as a result without requiring any manually crafted rules or heuristics.

==> sec_relatedworks.tex <==
\vspace{-1.9em}
\section{Related Works}
\label{sec:related_works}
\vspace{-1em}
%
%We divide the large body of research that is related to our work into the following broad categories.
%
\noindent\textbf{Scheduling}:
A large body of work focused on scheduling data-driven applications, long running user-facing services, ML-services etc. on multi-tenant commodity clusters covering various aspects such as: fairness of resource sharing~\cite{parkes2015beyond, ghodsi2013choosy, ghodsi2012multi, joe2013multiresource, popa2012faircloud, ghodsi2011dominant, grandl2015multi}, tail-latency optimization~\cite{suresh2015c3, ren2015hopper, ferguson2012jockey, leverich_eurosys2014, mace2015retro, bobtail, haque2015few} and on how to protect latency sensitive application while improving cluster utilizations~\cite{agarwal2012re, smite, paragon, quasar, borg, heracles, bubble_flux, bubble_up, q-clouds, omega, apollo}. This are distinct from our work as none of these scheduler attempt to self-learn the best scheduling strategy by discovering
hidden characteristics and dependence among applications. However, some of the proposed techniques (e.g. cycle-per-instruction~\cite{cpi2}) can be used with our technique to further fine-tune reward/penalty design.
%In the high performance computing (HPC) environment is different as no virtualization is used due to performance implications and schedulers~\cite{staples2006torque, hovestadt2003scheduling} do not handle long running or user-facing services or cron jobs.
%In monolithic schedulers like Docker-Swarm~\cite{docker-swarm}, Borg~\cite{borg}, Kubernetes~\cite{kubernetes}, typically all scheduling requests are handled by a single scheduling-agent that implements a generic scheduling algorithm. Thus it becomes difficult to use different scheduling logic depending on job types due to increased complexities. 
%Even though we use a single RL-agent for scheduling, it improves upon traditional monolithic scheduler by self-learning how different job types should be handled differently.
%Two-level schedulers such as Mesos~\cite{mesos} and YARN~\cite{yarn} separate the concerns of resource allocation and job placement and placement logic can be tailored towards specific applications.
%
%
%\vspace{0.1em}
%\noindent\textbf{Container Orchestration:}
%In monolithic schedulers like Docker-Swarm~\cite{docker-swarm}, Borg~\cite{borg}, Kubernetes~\cite{kubernetes}, typically all scheduling requests are handled by a single scheduling-agent that implements a generic scheduling algorithm. Thus it becomes difficult to use different scheduling logic depending on job types due to increased complexities. 
%Even though we use a single RL-agent for scheduling, it improves upon traditional monolithic scheduler by self-learning how different job types should be handled differently. Two-level schedulers such as Mesos~\cite{mesos} and YARN~\cite{yarn} separate the concerns of resource allocation and job placement and placement logic can be tailored towards specific applications. Media~\cite{medea_eurosys2018} is a two-level scheduler that optimizes placement of long-running-applications. However, such application-level schedulers lacks the global view of the cluster resulting in limited placement options ability to detect interference from running workloads that may degrade resource quality. 
%
%In Mesos, resources are offered to application-level schedulers, while YARN allows the application-level schedulers to request resources.
%Media~\cite{medea_eurosys2018} is a two-level scheduler that optimizes placement of long-running-applications. 
%However, such application-level schedulers lacks the global view of the cluster resulting in limited placement options ability to detect interference from running workloads that may degrade resource quality. 
%Moreover, the offer/request based interface to the scheduler can easily become quite complex to capture all possible aspects of the applications. Our approach, being monolithic, can detect possible resource competition that might lead to interference and more importantly, our self-learning RL-agent avoids configuration complexities. 
%\vspace{0.1em}
%\noindent\textbf{Virtual machine (VM) placement}:
%A large body of work also looks at VM placement and scheduling~\cite{rc-sosp-2017, vanga-eurosys-2018, ahn-hotcloud-2012, kim-VEE-2009, meng-infocom-2010, ghribi-ccgrid-2013, beloglazov-ccgrid-2010, gong2010press, novakovic2013deepdive, padala2009automated}. This is a related but slightly different problem as VMs can host a set of different applications/task inside it. Moreover, high-level of resource isolation and vartualization overhead makes the resultant resource usage footprint noisy, less repetitive and difficult to learn from. On the other-hand micro-services running inside container often show very clear and distinct characteristics and repetitive or long-running services makes it amenable to self-learning based scheduling.
%\vspace{0.1em}
%\noindent\textbf{Resource Isolation}:
%
%Several works focus on resource isolation techniques~\cite{cpi2, kim2009, gupta2006, xie2009, qureshi2006, kasture2014ubik, hsu2006communist, ebrahimi2010, muralidhara2011, jeyakumar2013, shieh2010, heracles}. 
%Heracles~\cite{heracles} uses all these aspects, albeit on the basis of Linux’s heuristic-driven scheduler.
%However, many of these techniques are still not available in the off the shelf machines that is used in most of datacenters due to several drawbacks. 
%Performance degradation due to interference is still a reality~\cite{leverich_eurosys2014, medea_eurosys2018, majiMiddleware, novakovic2013deepdive} 
%and we can never assume perfect isolation in multi-tenancy.
%Thus, our work is orthogonal to these works as it attempts to \textit{learn}
%the best scheduling strategy in the presence of imperfect isolation and complex workload patterns.

%\vspace{0.1em}
\noindent\textbf{Reinforcement Learning:}
Apart from DeepRM~\cite{deeprm} that we discussed in detail in Sec.~\ref{sec:background}, RL has been used in variety of scenarios including 
learning complex games~\cite{mnih2013playing, gibney2016google, lample2017playing}, robotics~\cite{mnih2015human, kaelbling1996reinforcement, kober2013reinforcement}, 
and very recently for video streaming~\cite{neural-abr-2017}, routing~\cite{boyan1994packet, valadarsky2017learning, mestres2017knowledge}, 
device placement~\cite{mirhoseini-icml-2017} etc.
%
%RL was used in offline setup for human resource scheduling for NASA shuttle missions~\cite{zhang1995reinforcement} where all inputs are known in advance while our setup requires online learning from job/service behavior.
%
%DeepRM~\cite{deeprm} is the closest to our work as it also attempts to learn online scheduling, but as mentioned in Section~\ref{sec:background}, cannot handle job placement decisions over multiple machines, does not capture interference between jobs and does not attempt to learn temporal patterns of the jobs to optimize placement. 



